Significance of Episodes Based on Minimal Windows

Discovering episodes, frequent sets of events from a sequence has been an active field in pattern mining. Traditionally, a level-wise approach is used to discover all frequent episodes. While this technique is computationally feasible it may result in a vast number of patterns, especially when low thresholds are used. In this paper we propose a new quality measure for episodes. We say that an episode is significant if the average length of its minimal windows deviates greatly when compared to the expected length according to the independence model. We can apply this measure as a post-pruning step to test whether the discovered frequent episodes are truly interesting and consequently to reduce the number of output. As a main contribution we introduce a technique that allows us to compute the distribution of lengths of minimal windows using the independence model. Such a computation task is surpisingly complex and in order to solve it we compute the distribution iteratively starting from simple episodes and progressively moving towards the more complex ones. In our experiments we discover candidate episodes that have a sufficient amount of minimal windows and test each candidate for significance. The experimental results demonstrate that our approach finds significant episodes while ignoring uninteresting ones.

==> algorithm.tex <==
\section{Computing the Distributions}
\subsection{Dependency Graph of Sub-episodes}

In order to compute the distribution $p_G$ for a given episode $G$ efficiently
we will compute it iteratively from certain sub-episodes. 

To be more precise, let $G$ be an episode and let $v \in \sinks{G}$ be a sink
node in $G$, then $G - v$ is a sub-episode of $G$ obtained by removing $v$ and
its related edges.

We define a closure of $G$, denoted by $\closure{G}$ to be
a set of $G$ and all sub-episodes obtained by iteratively removing sinks, that
is, we define $\closure{G}$ recursively
\[
	\closure{G} = G \cup \set{H \in \closure{G - v} \mid v \in \sinks{G}}.
\]
Note that, even though being a trivial pattern, the empty episode $\emptyset
\in \closure{G}$. Also note that if an episode has several sinks with the same
label, then removing different sinks may induce the same sub-episode. In this
case, we keep only one of these sub-episodes.

We define a directed graph $F_G = \pr{V(F_G), E(F_G)}$, whose nodes are the
episodes included in the closure of $G$, $V(F_G) = \closure{G}$. An edge $e =
(X, Y) \in E(F_G)$ with a label $a = \lab{e}$ exists if and only if $X \in
\sub{Y; a}$ In other words, there should be an edge between an episode and an
episode obtained by removing a sink node with a label $a$.

\subsection{Dependency Graph as Finite State Machine}

It will be useful to interpret the dependency graph $F_G$ as a finite state
machine $M$.  In fact, if we think $\emptyset$ as a starting state and $G$ as
an accept state, then the sequence $s$ covers $G$ if and only if there is a
sequence $t = \enset{s_{i_1}}{s_{i_N}}$ which $M$ accepts.

It will be useful to us to work directly with finite state machines. In order
to do that we wish to extend the definition of coverage and minimal windows to
the states of finite state machine. Let $M$ be a DAG representing a (possibly
non-deterministic) finite state machine and let $v$ be a state in $M$. We say
that $s$ covers $v$ if there is a sequence $t = \enset{s_{i_1}}{s_{i_N}}$ such
that $v$ can be reached  when $t$ is given to $M$ as an input. In that case we
set $\cover{s ; v, M} = 1$, and $0$ otherwise. We will ignore $M$ from the
notation if it is clear from the context.  Similarly we define $\mw{s ; v, M}$,
when $s$ covers $v$ but $s[2, L]$ and $s[1, L - 1]$ does not cover $v$.

\begin{lemma}
\label{lem:subepisode}
Let $M$ be a DAG representing a finite state machine and let $v$ be a state in
$M$. Let $s = \enpr{s_1}{s_L}$ be a sequence.

The sequence $s$ is a minimal window for $v$ if and only if the following
conditions are met:
\begin{enumerate}
\item There is an edge $e = (w, v)$ is an edge in $M$ with $\lab{e} = s_L$ such that $s[1, L - 1]$ covers $w$.
\item If $f = (u, v)$ is an edge in $M$ with $\lab{f} = s_L$, then $s[2, L - 1]$ does not cover $u$.
\item $s[1, L - 1]$ does not cover $v$.
\end{enumerate}
\end{lemma}

\begin{IEEEproof}
Assume that $s$ is the minimal window. The second and the third contidions are
trivial since the opposite would imply that there is a proper sub-sequence
covering $v$. Also by definition, $v$ must be visited through some edge, say
$e$.  The third condition now states that visiting must happen with the last
symbol $s_L$, thus $\lab{e} = s_L$.

To prove the opposite direction assume that the conditions are true.  It is
obvious from the first condition that $s$ covers $v$. Let $s[i, j]$ be a
minimal window for $v$. The third condition implies that $j = L$. The second
condition now implies that $i = 1$.
\end{IEEEproof}




\subsection{Computing the Distribution from a Stream}

Given a long stream $s$ our goal is to compute the empirical distributions
$q_G$ for a given set of episodes $\efam{G}$. In order to do that we extend our
definition of $F_G$ to the set of episodes. First we define $V(F_{\efam{G}}) =
\closure{\efam{G}} = \bigcup_{G \in \efam{G}} \closure{G}$. There is a labeld
edge $(X, Y)$ in $E(F_{\efam{G}})$ if $X$ can be otained from $Y$ by deleting a
sink with the same label.


For each episode $X$ in $V(F_\efam{G})$ we assign an index $\ind{X}$ to be the
index of the last discovered minimal window. When inspecting the symbol $s_i$
we check all edges in $e = (X, Y) \in E(F_G)$ for which $\lab{e} = s_i$. We
claim that $\ind{X} > \ind{Y}$ if and only if $[\ind{X}, i]$ is the minimal
window for $Y$.

The algorithm using this property is given in Algortihm~\ref{alg:stream}.
The next theorem uses Lemma~\ref{lem:subepisode} in order to prove that the
algorithm is correct.

\begin{algorithm}[htb!]
\begin{algorithmic}
\STATE Construct graph $F_\efam{G}$.
\STATE $\ind{X} \define 0$ for each episode $X \in V(F_\efam{G})$.
\FOR{$i = 1, \ldots L$}
\STATE $\ind{\emptyset} \define i$.
\FOR{$e = (X, Y) \in E(F_G), \, \lab{e} = s_i$}
\IF{$\ind{X} > \ind{Y}$}
\STATE $\ind{Y} \define \ind{X}$.
\ENDIF
\ENDFOR
\STATE Report minimal window $[\ind{Y}, i]$ for $Y$ if $\ind{Y}$ has changed.
\ENDFOR
\end{algorithmic}
\caption{An algorithm discovering all the minimal windows for episodes in
$\closure{\efam{G}}$ from the stream $s = \enpr{s_1}{s_L}$.}
\label{alg:stream}
\end{algorithm}

\begin{theorem}
The windows discovered by Algortihm~\ref{alg:stream} are the minimal windows for
$G$.
\end{theorem}

\begin{IEEEproof}
We will prove the theorem using induction over $i$. Assume that the algorithm is
correct for $s_1, \ldots s_{i - 1}$.

Assume that there is a minimal window $[j, i]$ for $G$. Interpret $F_G$ as a
finite state machine and let $e = (X, G)$ be the edge given in
Lemma~\ref{lem:subepisode}. Note that we have $\lab{e} = s_L$.  The first
condition of Lemma~\ref{lem:subepisode} and the induction assumption now imply
that we have $\ind{X} = j$. The second condition implies that $\ind{X}$ is the
largest among the parent nodes of $G$.  The third condition and the induction
assumption now imply $\ind{G} < \ind{X}$, hence the algorithm reports the
window.

To prove the other direction assume that at symbol $s_i$ we have $\ind{G} <
\ind{X}$, and that for any parent node $Y$ of $G$, we have $\ind{X} \geq
\ind{Y}$. Surely, by the induction assumption $s[\ind{X}, i - 1]$ covers $X$
and $s[\ind{X} + 1, i - 1]$ does not cover any parent node $Y$. Since $\ind{G}
< \ind{X}$ it follows that $s[\ind{X}, i - 1]$ cannot cover $G$.
Lemma~\ref{lem:subepisode} implies that $[\ind{X}, i]$ is a minimal window
for $G$.
\end{IEEEproof}

We should point out that the order in which the edges are iterated in
Algorithm~\ref{alg:stream} matters. Since $F_G$ is an asyclic graph, the nodes
have topological order. When visiting an edge $e = (X, Y)$ we should make sure
that we have already visited all edges $f = (U, V)$, where $V$ is a child of
$Y$.

Note that Algorithm~\ref{alg:stream} does not only output minimal windows for
$G$ but also for each sub-episode in $\closure{G}$.


\subsection{Computing Independence Model}
Our next goal is to compute $p_G(k)$ for a sequence of independent symbols.  We
compute the distribution by progressing iteratively through states in a finite
state machine.

In order to do that, let $G$ be an episode and let $M$ induced from $F_G$.  For
the moment we will make an assumption that for each state there is no two
incoming edges having the same label. This is certainly true for $F_G$ when
there is no multiple labels in $G$. We will deal with more general case later
on. 

The machine induced from $F_G$ has an important property which does not hold
for general finite state machines. 
\begin{lemma}
Let $M$ be the machine induced from $F_G$. Let $v$ be the state in $M$ and let $w$
be a parent state of $v$. If $s$ covers $v$, then $s$ covers $w$ also.
\label{lem:child1}
\end{lemma}

\begin{IEEEproof}
Let $X$ be the episode represented by the state $v$ and let $Y$ be the episode
represented by the state $w$. If $v$ covers $s$, then it must cover $X$. Since
$Y$ is an episode obtained from $X$ by removing one sink, $s$ also covers $Y$
and thus cover $w$.
\end{IEEEproof}

Let $v$ be a state in $M$ and let us write $r(s; v) = \cover{s; v} -
\cover{s[2, L]; v}$. Thus $r(s; v) = 1$ if and only if $s$ covers $v$ but $s[2,
L]$ does not.

We also define $n(s; v)$ to return binary value such that $n(s; v) = 1$ if and
only if there is $i$ such that $s[1, i]$ is a minimal window for $v$. Note that
this implies
\begin{equation}
p\fpr{n(s; v) = 1} = \sum_{i = 1}^L p\fpr{\mw{s[1, i]; v} = 1}.
\label{eq:ident1}
\end{equation}

\begin{proposition}
\label{prop:mw}
Let $s = \enpr{s_1}{s_k}$ be a random sequence of length $k$ and let $t = s[1,
k - 1]$. Then we have
\[
\begin{split}
	&p\fpr{\mw{s; v}} \\
	&\quad = \sum_{e = (w, v) \in E(M)} p\fpr{\lab{e}}\fpr{p\fpr{r(t; w)} - p\fpr{n(t; v}}.
\end{split}
\]
\end{proposition}


\begin{IEEEproof}
Since $v$ has incoming edges with unique labels Lemma~\ref{lem:subepisode}
states that $s$ is a minimal window for $v$ if and only if there is an edge $e
= (w, v)$ with $\lab{e} = s_k$ such that $t$ covers $w$ but $t[2, k - 1]$ does
not, that is, $r(t; w) = 1$, and also $t$ does not cover $v$.

Note that if we have $t$ for which $r(t; w)$, then
Lemma~\ref{lem:child1} implies that $t[2, k - 1]$ cannot cover $v$. Hence $t$
covers $v$ if and only there is a minimal window for $v$ starting from $s_1$,
that is, $n(t; v) = 1$. This proves the statement.
\end{IEEEproof}


If we assume that we know $p\fpr{r(t; w)}$, we can iteratively compute
$p\fpr{\mw{s; v} = 1}$ and $p\fpr{n(s; v) = 1}$ by using
Proposition~\ref{prop:mw} and Eq.~\ref{eq:ident1} in turns.

The following proposition tells us how to compute $r$ from $c$.
\begin{proposition}
\label{prop:r}
Let $s = \enpr{s_1}{s_k}$ be a random sequence of length $k$ and let $t = s[1,
k - 1]$. Then we have
\[
\begin{split}
	&p\fpr{r(s; v)} \\
	&\quad = \sum_{e = (w, v) \in E(M)} p\fpr{\lab{e}}\fpr{p\fpr{c(t; w)} - p\fpr{c(t; v}}.
\end{split}
\]
\end{proposition}
\begin{IEEEproof}
By definition, we have
\[
p\fpr{r(s; v)} = p\fpr{\cover{s; v}} - p\fpr{\cover{u; v}},
\]
where $u = s[2, k]$. Since $p\fpr{\cover{u; v}} = p\fpr{\cover{t; v}}$, we
conclude that $p\fpr{r(s; v)}$ is the probability of sequence $s$ covering $v$
but $s[1, k - 1] = t$ not covering it. This implies that $s_k$ must have the label
of one of the sinks, that is, there is an edge $e =(w, v)$ with $\lab{e} =
s_k$. We also must have that $t$ covers $w$ but not $v$. Note that
this probability can be written as
\[
p(\cover{s; w}) - p(\cover{t; w}, \cover{t; v}) = p(\cover{s; w}) - p(\cover{t; v}),
\]
where the equality follows from Lemma~\ref{lem:child1}.
\end{IEEEproof}


All the preceeding calculations are valid only if there is no multiple incoming
edges with the same label. However, if an episode has multiple nodes with
the same label, then $F_G$ may violate our assumption. Hence, we cannot
directly use it as our finite state machine accepting $G$. Luckily, we can
modify $F_G$ so that it satisfies our requirement. Let $M$ be the machine
corresponding to $F_G$. Consider a machine in which we have reversed the
directions of all the edges. If we had multiple incoming edges with identical
label in $F_G$, this implies that the reversed machine is non-deterministic.
Use the standard technique to transform a non-deterministic finite state
machine into a deterministic one. Finally, switch back the directions of the
edges. This new machine, say $M'$ will accept $s$ if and only if $M$ accepts
$s$ and every incoming edge has a unique label.

To give a more explicit definition, we can define $M'$ iteratively. A state $v$
in $M'$ corresponds to a set of episodes $\mathcal{X} = \enset{X_1}{X_N}$. Let
$x$ be a sink in one of $X_i$ having the label $a$. Then there exists a state
$w$ that corresponds to the set of episodes $\mathcal{Y} = \enset{Y_1}{Y_M}$
such that
\[
\mathcal{Y} = \pr{\bigcup_{X \in \mathcal{X}} \sub{X; a}} \cup \set{X \in \mathcal{X}; \sub{X} = \emptyset},
\]
that is, each $Y \in \mathcal{Y}$ is either a copy of $X \in \mathcal{X}$ if
$X$ has no sinks with a label $a$, or $Y$ is obtained from $X$ by removing a
sink.  An edge from $w$ to $v$ has a label $a$. 

In order to make Propositions~\ref{prop:mw}--\ref{prop:r} valid for $M'$, we
need to make sure that Lemma~\ref{lem:child1} holds also for $M'$.  The
following two lemmas will prove that it is indeed the case.

\begin{lemma}
Let $M'$ be the machine constructed from the machine induced from $F_G$. Let
$v$ be the state in $M'$. Let $\enset{X_1}{X_N}$ be the set of episodes
represented by $v$.  The $s$ covers $v$ if and only if $s$ covers at least one $X_i$.
\end{lemma}

\begin{IEEEproof}
We will prove this by induction. Assume that the lemma holds for all parent
states of $v$.

Assume that $s$ covers $v$.  Let $t$ be sub-sequence of $s$ that leads $M'$
from $\emptyset$ to $v$.  Let $s_e$ be the last symbol of $s$ occuring in $t$.
There is a parent state $w$ which $s[1, e - 1]$ covers. Let $\enset{Y_1}{Y_M}$
be the episodes represented by $w$. By the induction assumption at least one
$Y_i$ is covered by $s[1, e - 1]$. If there is $X_j = Y_i$, then $X_j$ is
covered by $s$, otherwise there is $X_j$ which obtained from $Y_i$ by adding a
sink with $s_e$ as a label. In this case $s$ covers $X_j$ also.

To prove the other direction assume that $s$ covers one $X_j$.  Let $f$ be the
function mapping each node in $X_j$ to an index of $s$. Let $e$ be the largest
index that $f$ may achieve, and let $x$ be the node for which $f(x) = e$. It
must be the case that $x$ is a sink of $X_j$, and hence there is an edge $(w,
v)$ having the label $s_e$. We must have $X_j - x$ in one of the episodes, say
$Y_i$. By the induction assumption $w$ is covered by $s[1, e - 1]$ and hence
$s[1, e]$ covers $v$.
\end{IEEEproof}

\begin{lemma}
Let $M'$ be the machine constructed from the machine induced from $F_G$. Let
$v$ be the state in $M'$ and let $w$ be a parent state of $v$. If $s$ covers
$v$, then $s$ covers $w$ also.
\label{lem:child2}
\end{lemma}

\begin{IEEEproof}
Let $X$ be the episode represented by $v$ and covered by $s$. Let $Y$ be the
sub-episode of $X$ in $w$. Since $s$ covers $Y$, $s$ also covers $w$.
\end{IEEEproof}

\begin{algorithm}
\begin{algorithmic}[1]
\STATE $M \define $ machine based on $F_G$ and having unique incoming edges for each state.
\STATE \COMMENT{Initialize probabilities.}
\FOR{$k = 0, \ldots K$.}
	\FOR{$v \in V(M)$}
		\STATE $c(k; v) \define 0$, $r(k; v) \define 0$. 
		\STATE $n(k; v) \define 0$, $\mw{k; v} \define 0$. 
	\ENDFOR
	\STATE $c(k, \emptyset) \define 1$.
\ENDFOR
\STATE \COMMENT{Compute $r$ and $c$.}
\FOR{$v \in V(M)$}
	\FOR{$k = 1, \ldots K$.}
		\FOR{$e = (w, v) \in E(M)$}
			\STATE $x \define c(k - 1; w) - c(k - 1; v)$.
			\STATE $r(k; v) \define r(k; v) + p\fpr{\lab{e}}x$.
		\ENDFOR
		\STATE $c(k; v) \define r(k, v) + c(k - 1; v)$.
	\ENDFOR
\ENDFOR
\STATE \COMMENT{Compute $m$ and $n$.}
\FOR{$v \in V(M)$}
	\FOR{$k = 1, \ldots K$.}
		\FOR{$e = (w, v) \in E(M)$}
			\STATE $x \define r(k - 1; w) - n(k - 1; w)$.
			\STATE $\mw{k; v} \define \mw{k; v} + p\fpr{\lab{e}}x$.
		\ENDFOR
		\STATE $n(k; v) \define \mw{k, v} + n(k - 1; v)$.
	\ENDFOR
\ENDFOR
\STATE \COMMENT{Compute $p_G$.}
\STATE $v \define$ accept state for $G$.
\STATE $N \define \sum \mw{k, v}$.
\FOR{$k = 1, \ldots K$.}
	\STATE $p_G(k) \define \mw{k; v} / N$
\ENDFOR

\end{algorithmic}
\caption{Algorithm for computing $p_G$, the distribution of minimal windows
under the independence assumption.}
\end{algorithm}

